The Groupon Effect on Yelp Ratings: A Root Cause Analysis

Daily deals sites such as Groupon offer deeply discounted goods and services to tens of millions of customers through geographically targeted daily e-mail marketing campaigns. In our prior work we observed that a negative side effect for merchants using Groupons is that, on average, their Yelp ratings decline significantly. However, this previous work was essentially observational, rather than explanatory. In this work, we rigorously consider and evaluate various hypotheses about underlying consumer and merchant behavior in order to understand this phenomenon, which we dub the Groupon effect. We use statistical analysis and mathematical modeling, leveraging a dataset we collected spanning tens of thousands of daily deals and over 7 million Yelp reviews. In particular, we investigate hypotheses such as whether Groupon subscribers are more critical than their peers, or whether some fraction of Groupon merchants provide significantly worse service to customers using Groupons. We suggest an additional novel hypothesis: reviews from Groupon subscribers are lower on average because such reviews correspond to real, unbiased customers, while the body of reviews on Yelp contain some fraction of reviews from biased or even potentially fake sources. Although we focus on a specific question, our work provides broad insights into both consumer and merchant behavior within the daily deals marketplace.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conc}

We have examined a number of hypotheses for explaining what we have
dubbed the Groupon effect.  While there remain challenges in trying
to exactly quantify the different issues at play, we have shown that a
combination of poor business behavior, Groupon user experimentation,
and an artificially high baseline all play a role.  

Our compilation of evidence about Groupon users, as presented in
Tables~\ref{tab:user-stats} and~\ref{tab:review-stats}, highlights
that on average, Groupon users provide detailed reviews that are
valued more highly by their Yelp peers.  Contrary to what some would
believe, the evidence suggests that Groupon users are no more critical
than their peers, although they may well be experimenting with a new
business when using a Groupon.  It seems odd that any business would
incur marketing costs only to treat new customers poorly, but as the 
FTD example shows, sometimes businesses do unusual things, such as
treating potential long-term customers as a sunk cost rather than as an
opportunity.  Although it seems obvious, we would advise businesses to
treat Groupon customers as well as (or possibly better than?) their
other customers to avoid negative reputational impact.


==> dataset.tex <==
\section{Datasets}
\label{sec:data}

Our data was collected from two websites: Groupon.com and Yelp.com. The Groupon 
data set consists of information about a set of \numGrouponDeals deals offered 
by Groupon in 20 major metropolitan areas in the US between January 3rd and 
July 3rd, 2011.

To collect Yelp data, we started from Groupon merchants with whom we
could confidently associate a corresponding Yelp page, through one of
the following two methods. First, we leveraged the fact that in many
cases, the Groupon offer page contains a direct link to the Yelp page
for the purpose of promoting the deal. Second, we used the search
feature on Yelp with the merchant name and merchant location, and when
the search resulted in an exact match, we used that association. In
many instances, by searching on Yelp, we found businesses whose name
and address only partially matched the corresponding business. Even
though the associations were likely correct in most cases, we chose to
ignore them. Through these two mechanisms, we successfully associated
\numGrouponBusinesses Groupon businesses, a set we refer to as our
\emph{seed set}.

We then proceeded to compile two datasets of reviews from
Yelp.com. For the first dataset (Dataset 1), our goal was to collect
the entire review histories of {\em all} reviewers who had ever
reviewed {\em any} of the businesses in the seed set prior to the
collection date, January 26th 2012. Our crawl left us with
\numGrouponReviewsComplete reviews for \numGrouponBusinessesComplete
distinct businesses. This dataset contains as a subset all reviews for
the \numGrouponBusinesses Groupon businesses in our seed set.

For the second dataset (Dataset 2), we restricted attention to the
review histories of the seed businesses (which constituted a subset of
the reviews in our first crawl). We separated reviewers in this set
into two groups: those that had never mentioned Groupon in any of
their reviews (\numNonGrouponReviewers reviewers), and those that had
mentioned Groupon at least once (\numGrouponReviewers reviewers). The
latter set of reviewers had reviewed \numGrouponReviewerOtherBusinesses businesses other than those in the
seed set.  We collected the complete review histories of a random
sample of \numGrouponReviewerOtherBusinessesSample of these businesses
(many of which have presumably never run a Groupon offer).

We note that Yelp algorithmically {\em filters} reviews based on
legitimacy and how ``established'' the reviews' authors are (see
\cite{yelp-filter} for details).  Filtered reviews do not count
towards Yelp ratings, and filtered reviews for a merchant are not
visible to users by default, although they can be accessed by solving
a CAPTCHA.  A review's status is not permanent: as users become more
or less established, their reviews can switch from being visible to
being filtered and vice-versa. Yelp purposefully avoids elaborating
precisely what factors determine how established users are and whether
reviews are filtered to limit fraud.

To be clear, review histories of {\em users} contain {\em both} their
filtered and their unfiltered reviews, and no indication is given as
to which reviews are filtered.  (To make this determination, one could
cross-check a review to see if it is visible on the {\em merchant}
page.)  Hence Dataset 1 contains filtered reviews, while our
methodology for Dataset 2 collected only those reviews that were not
filtered at the time of collection.





==> intro.tex <==
\section{Introduction}


Groupon is the largest of the daily deals businesses: each day, in a
number of markets (generally cities), they offer Groupons, which are 
deals providing a coupon for some product or service at a substantial
discount, generally approximately 50\% off the list price.  Daily deal
sites such as Groupon represent a novel approach to Internet marketing
that tap into local markets, and based on the massive scale and rapid 
growth of such sites, the business model is worthy of further 
examination. 

In previous work examining Groupon, we measured and evaluated aspects
of Groupon's operational strategy, as well as observed the impact of customer behaviors
including word-of-mouth effects and how running a Groupon offer 
affects a merchant's reputation~\cite{OurGroupon}.  One specific finding that 
received significant interest and attention was that Yelp reviews that
contained the word ``Groupon'' provided, on average, significantly lower
ratings than reviews that did not, to the extent that it significantly
lowered the average rating for businesses that used Groupon.  In the
original paper, we did not examine reasons to explain this finding,
leaving it to future work.  Our analysis met with a variety of
reactions, ranging from disbelief, to a number of plausible explanations for
why this phenomenon should be expected: for example, Groupon users are
fussy reviewers, Groupon businesses provide worse service than their peers, 
businesses discriminate by providing worse service specifically to Groupon 
customers, and Groupon users are less of a good fit for the businesses 
where they redeem Groupons.  

In this paper, we return to our finding of a sharp decline in Yelp ratings 
scores that coincides with Groupon offers, a phenomenon we term the 
{\em Groupon effect}, and consider possible explanations through the lens of data 
analysis, based on an extensive dataset we gathered from Groupon and Yelp.  
Through this undertaking, we learn significantly more about the daily deals model, 
including the behavior of Groupon users and businesses.  A priori, one or more of
the suggested explanations might be valid, and as such we examine
where data provides positive and negative evidence for each.

However, we also suggest and provide evidence for an alternative
explanation that we have not heard previously.  It is well known that
a potential problem with review sites is that businesses may actively
solicit positive reviews for their business, either through
unscrupulous means such as hiring people to write positive reviews for
them, or by less questionable means such as encouraging reviews from
obviously enthusiastic customers.  (In some cases, they may also
attempt to place negative reviews for their competitors, although this
is arguably a less effective strategy.)  Indeed, Yelp filters its
reviews to prevent ``spam reviews'' from affecting its ratings.  

Our hypothesis is that one reason for the discrepancy in review scores
is that reviews that mention Groupon correspond almost exclusively to
reviews written by actual customers who use the service, and that
other reviews are significantly more likely to be ``fake'' or otherwise
introduced in an arguably artificial manner.  Hence, we suggest
that, at least in part, the issue is not that reviews mentioning
Groupon are somehow unusually low, but that the baseline of other
reviews are on average artificially high, most likely because of
actions taken by businesses designed specifically to generate
high-scoring reviews.

As part of our analysis efforts, we utilize a new tool for the study of
the relationship between reviews and daily deal sites, namely an
ordered probit analysis.  Such analyses are used in regressions where
the output variable is a ranked score from a finite domain, as in
reviews.  These regression analyses provide statistical backing for
our higher-level thoughts and discussions, for which we often utilize
more easily interpreted plots and graphs.  Such methods have been used
in other economic analyses, including in problems of adverse
selection, which bear some similarity to our setting -- by using
Groupon as a matchmaker, businesses may be targeting customers 
from a less-than-ideal population, and similarly, customers are 
incented to select businesses from a smaller population.  In both
cases, customers and businesses are operating with incomplete information 
about each other.  

After discussing related work (\S~\ref{sec:relwork}), and explaining 
our datasets and terminology (\S~\ref{sec:data}), we begin our paper by
examining the evidence for the Groupon effect 
using extensive new data beyond that originally presented in our prior
work (\S~\ref{sec:effect}).
We then turn to various plausible explanations in \S~\ref{sec:whodunit}, 
including our hypothesis regarding an excessively high baseline, and consider
the evidentiary information we have to support or refute them.  Along the way,
various insights into Groupon, Yelp, and the interactions between these two
firms arise naturally.  We then deepen our analysis by interpreting our data 
using mathematical models and regression in \S~\ref{sec:model} to pinpoint the
contributing factors to the Groupon effect from key consumer-specific, merchant-specific, and review-specific attributes
before concluding in \S~\ref{sec:conc}.
 



==> notation.tex <==
\subsection{Terminology}
\label{sec:notation}

We employ the following terminology to describe certain aspects of our dataset
in the paper.  We use the term \emph{Groupon business} to refer to any merchant
that ran a Groupon deal in our seed set. We will use the term 
\emph{Groupon review} to refer to any Yelp review for a Groupon business that 
contains the word ``Groupon'' in its text and we will call the author of 
one or more such reviews a \emph{Groupon user}. We will use the 
terms \emph{non-Groupon business}, \emph{non-Groupon review}, 
and \emph{non-Groupon user} to refer 
to the corresponding complementary sets.

A review on Yelp.com consists of a star rating, and some free text. The star rating
takes on a value from $\{1,2, 3, 4, 5\}$.  
For each Groupon business, we associate an offer date that
corresponds to the date they initiate a Groupon offer.  Then, for every 
review of a Groupon business, we associate an integer offset  with
that review reflecting how many days after (or before) the offer date the
review was posted.  For example, a review posted on March 7th for a business
that subsequently initiates a Groupon offer on March 13th would have an offset
of -6.


==> related.tex <==
\section{Related Work}
\label{sec:relwork}

Our present work relates to multiple lines of research.  First, there
are a small number of recent works examining daily deal sites such as
Groupon, including data analysis and models of user and business
behavior.  Second, past research on coupons is relevant, as a Groupon
can naturally be thought of as a type of coupon.  There are fairly
substantial differences, however, between Groupons and traditional
coupons; for example, Groupons require an up-front purchase, and they
are incorporated into various social networks -- one can ``like'' a
Groupon deal on Facebook.  Third, there are a significant number of
papers on online review sites, covering themes such as how reviews
impact purchase decisions and how reviewers' behavior can be affected
by previous reviews.  However, there appear to be few papers studying
the type of interactions between major economic agents -- in this case
daily deal sites and review sites -- that we examine here.  
As the literature on coupons and reviews related to our work is
extensive, space requirements necessitate limiting ourselves to a brief discussion
of relevant papers here.

The question of how daily deal sites affect the reputation of a business, and 
the idea of using Yelp reviews as a proxy, was initiated in \cite{OurGroupon}. 
Other previous works, however, had initiated studies of daily deal sites more 
generally, focusing primarily on the question of whether such deals would be 
profitable for businesses, without considering 
reputation~\cite{Arabshahi2010Undressing,Dholakia2010How, Edelman2010To}. 
Merchant reputation in the context of Yelp reviews has also been separately 
considered~\cite{Luca2011}.

Somewhat surprisingly, we have not found work that directly
shows that coupon users provide worse reviews on online review forums
or other review settings.  However, there is general work on the issue
of marketing efforts bringing in unprofitable customers (see, e.g.,
\cite{cao2005reducing} and references therein); this can be viewed as an
adverse selection problem, where marketing efforts bring in the
wrong kind of customer instead of profitable new customers.  It seems
reasonable to extend this line of thinking to encompass the
possibility that Groupons may bring in customers that provide less of 
a fit, and thereby worse reviews, to merchants using Groupon. 

Other relevant work on coupons includes analysis that shows that customers 
frequently redeem coupons just before the expiration date \cite{inman1994}, a 
useful fact that we observe in our data. Previous work showing that 
coupons distributed through mass media induce brand switching and reduce loyalty 
\cite{dodson1978impact,shaffer1995competitive} is also relevant to our study. 

There has been extensive work studying online review sites that
relates to our study.  For example, \cite{chevalier2003} discusses
analysis of book review sites showing that review features such as
length are important to potential customers, not just the average star
rating;  we examine length and other features of Yelp reviews here as well.  
Recent work shows that online review scores tend to decline over time
\cite{godes2011sequential},
an issue we take into account in our analysis.  Related work suggests
that over time, there may be a tendency for reviews to take on extreme
values \cite{wu2008public,dellarocas2006statistical}.  

Additionally, our work makes use of a generalized ordered probit model 
\cite{terza1985ordinal} for the regression of Yelp ratings on their 
characteristics. Both the generalized and the standard ordered probit model 
\cite{McKelvey75} have been used extensively to model ordinal outcomes from 
cattle characteristics \cite{sy1997estimating} to stock prices 
\cite{hausman1992ordered}.


==> tables/biprobit-groupon-mention.tex <==

\begin{table*}[t]
\begin{centering}
\tbl{Predicted probabilities for the bivariate probit regression (Equation 
\ref{eqn:biprobit-exp}).}{
\begin{tabular}{cccrccc}
\toprule
Groupon user & Groupon mention && 
$(Y_{cat}, Y_{zip})=$ 
(1, 1) &
(1, 0) &
(0, 1) &
(0, 0) \\
\cline{1-2} \cline{4-7}
False &   False && 38.49\% & 15.65\% &14.54\% &31.30\% \\[1ex]
True  &   False &&  66.92\% & 14.05\% &9.09\% &9.23\% \\[1ex]
True  &   True  && 34.73\% & 15.77\% & 14.13\% & 35.35\% \\
\bottomrule
\end{tabular}
}
\label{tab:biprobit-groupon-mention-pr}
\end{centering}
\end{table*}





==> tables/biprobit-long.tex <==
\begin{table*}[t]
\begin{centering}
\tbl{Estimates for the bivariate probit regression 
(Equation~\ref{eqn:biprobit-exp}) on Yelp matching category and ZIP. Log-likelihood 
-223024.8, AIC 446199.7, $\rho$ = 0.31 (Std. Err. 0.003). Business city and 
category coefficients are omitted for brevity.}{
\begin{tabular}{p{5cm} r r r c r r r}
\toprule
% & \multicolumn{7}{c}{\text{probit}($\text{Pr}[Y_{cat}=1, Y_{zip}=1])$)} \\ [1ex]
% \cline{2-8}
& \multicolumn{3}{c}{Matching category} && \multicolumn{3}{c}{Matching ZIP}\\
& \text{Est.} & \text{Std. Err.}  & $t$\text{-value} && \text{Est.} & \text{Std. Err.}  & $t$\text{-value}\\
\cline{2-4} \cline{6-8}
(Intercept) & -0.46 & 0.02 & -18.94 && -0.18 & 0.02 & -7.83 \\  [1ex]
Groupon user  & 0.11 & 0.01 & 11.48 && 0.05 & 0.01 & 6.09 \\ [1ex]
Groupon mention & -0.10 & 0.02 & -6.13 && -0.10 & 0.01 & -6.57 \\ [1ex]
log(Review count) & 0.58 & 0.002 & 231.64 && 0.45 & 0.002 & 204.53 \\ 
\bottomrule
\end{tabular}
}
\label{tab:biprobit-groupon-mention}
\end{centering}
\end{table*}




==> tables/business-reviews-stats-table.tex <==
\begin{table*}[b]
\begin{centering}
\tbl{Summary statistics of reviews of Groupon businesses. Means and standard deviations (in parentheses).}{
\begin{tabular}{ccccccccr}
\toprule
\multirow{2}{*}{Groupon user} 
& \multirow{2}{*}{Groupon mention} 
& & &
\multicolumn{3}{c}{Votes} &
& 
\\
\cline{5-7}
&&&
\multicolumn{1}{c}{Length} & 
\multicolumn{1}{c}{Funny} & 
\multicolumn{1}{c}{Useful} & 
\multicolumn{1}{c}{Cool} & 
\multicolumn{1}{c}{Stars} & 
Count \\ 
\cline{1-2}\cline{4-9}
False &   False && 715.15 & 0.23 & 0.51 & 0.27 & 3.76 & 176,653 \\ 
\multicolumn{2}{c}{(\emph{Reviewer has never mentioned Groupon})}  && (608.96) & (1.30) & (1.74) & (1.21) & (1.24) &  \\  [1ex]
True &  False && 881.01 & 0.62 & 1.19 & 0.73 & 3.68 & 37,453 \\
\multicolumn{2}{c}{(\emph{Groupon user, mentioned Groupon elsewhere})}  && (662.49) & (2.21) & (2.66) & (2.12) & (1.09) &  \\  [1ex]
True &   True && 1109.48 & 0.37 & 1.11 & 0.37 & 3.28 & 13,602 \\ 
\multicolumn{2}{c}{(\emph{Groupon user, mentioned Groupon})}   && (771.17) & (1.43) & (2.80) & (1.34) & (1.40) &  \\ 
\bottomrule
\end{tabular}
}
\label{tab:review-stats}
\end{centering}
\end{table*}

% NM: Never mention & 738 (617) & 0.33 & 0.69  & 0.38  & 3.75 (1.22) & 202,663 \\ 
% MG: Mention Groupon  & 1111 (766) & 0.44  & 1.33  & 0.44 & 3.28 (1.40) & 12,805 \\ 
% ME: Mention elsewhere  & 910 (679) & 0.73 & 1.43  & 0.89 & 3.67 (1.08) & 14,984 \\ 

%%  More detailed data.
%No & No & 737.51 (616.87) & 0.33 (1.58) & 0.69 (2.02) & 0.38 (1.46) & 3.75 (1.22) & 202,663 \\ 
%No & Yes & 910.15 (678.32) & 0.73 (2.09) & 1.43 (2.74) & 0.89 (2.23) & 3.67 (1.08) & 14,984 \\ 
%Yes & Yes & 1111.09 (766.35) & 0.44 (1.59) & 1.33 (3.02) & 0.44 (1.50) & 3.28 (1.40) & 12,805 \\ 


==> tables/deltas-by-category-table.tex <==
\begin{table}[t]
\begin{centering}
\tbl{Changes in ratings around the Groupon offer date by category for categories with at least 100 deals.}{
\begin{tabular}{lrc}
\toprule
 & \multicolumn{2}{c}{Change in Rating} \\
 & Mean & Std. Dev. \\
\cline{2-3}
Arts and Entertainment & -0.05 & 1.03 \\ 
Automotive & -0.34 & 1.28 \\ 
Beauty \& Spas & -0.28 & 1.15 \\ 
Education & -0.16 & 1.02 \\
Food \& Drink & -0.25 & 0.87 \\ 
Health \& Fitness & -0.13 & 1.03 \\ 
Home Services & 0.42 & 1.65 \\
Nightlife & -0.03 & 0.71 \\ 
Pets & 0.09 & 1.36\\
Professional Services & -0.39 & 1.28 \\ 
Restaurants & -0.18 & 0.75 \\ 
Shopping & -0.23 & 1.17 \\ 
Travel & -0.13 & 0.88 \\ 
\bottomrule
\end{tabular}
}
\label{tab:deltas-by-category}
\end{centering}
\end{table}


==> tables/experimentation-table.tex <==
\begin{table*}[t]
\begin{centering}
\tbl{Summary statistics of customer experimentation.}{
\begin{tabular}{cccccccc}
\toprule
\multirow{2}{*}{Groupon user} 
& \multirow{2}{*}{Groupon mention} 
&& \multicolumn{2}{c}{Category match?} 
&& \multicolumn{2}{c}{ZIP match?} \\
&&& Yes & No && Yes & No\\
\cline{1-2} \cline{4-5} \cline{7-8}
False & False  && 70\% & 30\% && 68\% & 32\% \\ [1ex]
True  & False  && 84\% & 16\% && 80\% & 20\% \\ [1ex]
True  & True  &&  67\% & 33\% && 66\% & 34\% \\ 
\bottomrule
\end{tabular}
}
\label{tab:experimentation-stats}
\end{centering}
\end{table*}


==> tables/filtered-reviews-table.tex <==
\begin{table*}[t]
\begin{centering}
\tbl{Percentage of filtered reviews for Groupon vs. non-Groupon users.}{
\begin{tabular}{cccrrcc}
\toprule
\multirow{2}{*}{Groupon user} & \multirow{2}{*}{Groupon mention} && \multicolumn{4}{c}{Reviews}\\
&&& Visible & Filtered & Filtered pct. & Avg. Rating \\
\cline{1-2} \cline{4-7}
False & False  && 4,837 & 723 & 14.95\% & 3.79\\ [1ex]
True  & False  && 6,496 & 707 & 10.88\% & 3.58 \\ [1ex]
True  & True   && 175  &  19 & 10.86\% & 3.28\\
\bottomrule
\end{tabular}
}
\label{tab:filtered-stats}
\end{centering}
\end{table*}


==> tables/groupon-vs-non-groupon-users.tex <==
\begin{table*}[t]
\begin{centering}
\tbl{Summary statistics of user profiles for Groupon users vs. non Groupon users. Means and standard deviations (in parentheses).}{
\begin{tabular}{lcccccr}
\toprule
                   & Yelping Since & Friends & Fans & Reviews & Firsts & Count \\ 
\cline{2-7}				   
Groupon user       & 2009-06-27 & 44.94 & 4.38 & 89.60 & 7.19 & 21,020 \\ 
                   & (506.18) & (144.28) & (16.74) & (160.34) & (29.40) &  \\ [3ex]
Not a Groupon user & 2009-06-01 & 24.43 & 1.92 & 44.25 & 3.72 & 127,946 \\ 
                   & (530.01) & (106.62) & (12.49) & (88.57) & (19.32) &  \\ 
\bottomrule
\end{tabular}
}
\label{tab:user-stats}
\end{centering}
\end{table*}

==> tables/johns-oprobit-table.tex <==
% This is the generalized ordered probit model with 3 Groupon periods:
% Pre-Groupon, Pre-Expiry, Post-Expiry

\begin{table*}[t]
\begin{centering}
\tbl{Coefficient estimates for the generalized ordered probit regression of 
Yelp ratings. Standard errors are shown in parentheses. Log-likelihood 
-316,365, AIC 632,846. Business city and category coefficients are 
omitted for brevity.}{
\begin{tabular}{p{4cm} r r r r}
\toprule
& \multicolumn{4}{c}{$\text{probit}(Pr[y_{ij}\le n])$}\\
& \multicolumn{1}{c}{n=1} 
& \multicolumn{1}{c}{n=2} 
& \multicolumn{1}{c}{n=3} 
& \multicolumn{1}{c}{n=4} \\ [1ex]
\cline{2-5}
(Intercept $\kappa_n$)    &       -1.48 (0.019) & -1.01 (0.018) & -0.49 (0.018) & 0.37 (0.018) \\ [1ex]
%%                          &       (0.01877) & (0.01844) & (0.01830) & (0.01830) \\  [1ex]
%						  
Groupon mention           &       -0.68 (0.017) & -0.54 (0.014) & -0.32 (0.013) & -0.13 (0.014) \\ [1ex] 
%%                          &       (0.01773) & (0.01443) & (0.01323) & (0.01441) \\  [1ex]
%
Groupon user              &       0.29 (0.012) & 0.13 (0.008) & -0.10 (0.008) & -0.28 (0.008) \\  [1ex]
%%                          &       (0.01226) & (0.00891) & (0.00750) & (0.00792) \\  [1ex]
%
During Groupon deal       &       -0.24 (0.009) & -0.17 (0.007) & -0.05 (0.007) & 0.06 (0.007) \\ [1ex]
%%                          &       (0.00944) & (0.00772) & (0.00692) & (0.00702) \\ [1ex]
%
Post Groupon deal         &       -0.19 (0.012) & -0.13 (0.010) & -0.05 (0.009) & 0.04 (0.009) \\ [1ex]
%%                          &       (0.01267) & (0.01038) & (0.00930) & (0.00953) \\  [1ex]
%
Review rank               &       3.8E-4 (3E-5) & 1.6E-4 (2E-5) & 0.9E-4 (2E-5) & 3.6E-4 (2E-5) \\ [1ex]
%%                          &       (0.00003) & (0.00002) & (0.00002) & (0.00002) \\ 
\bottomrule
\end{tabular}
}
\label{tab:oprobit-model}
\end{centering}
\end{table*}


==> tables/margeff-table-periods.tex <==
\begin{table*}[t]
\begin{centering}
\tbl{Average marginal effects of the explanatory model variables on probalities of receiving a specific Yelp rating.}{
\begin{tabular}{p{4cm} rrrrr}
\toprule
 & \multicolumn{5}{c}{\text{Yelp rating}}\\
%\cline{2-6}
 & \multicolumn{1}{c}{1}
 & \multicolumn{1}{c}{2} 
 & \multicolumn{1}{c}{3} 
 & \multicolumn{1}{c}{4} 
 & \multicolumn{1}{c}{5} 
 \\
\cline{2-6}
Groupon mention      &   10.223\% & 3.802\% & -2.242\% & -7.388\% & -4.394\% \\ [1ex]
Groupon user         &   -4.436\% & 1.095\% & 6.544\% & 6.398\% & -9.601\% \\  [1ex]
During Groupon deal  &    3.577\% & 0.778\% & -2.544\% & -4.017\% & 2.206\% \\  [1ex]
Post Groupon deal    &    2.791\% & 0.575\% & -1.737\% & -3.069\% & 1.440\% \\  [1ex]
Review rank          &   -0.006\% & 0.002\% & 0.008\% & 0.010\% & -0.013\% \\  
\bottomrule
\end{tabular}
}
\label{tab:margeff}
\end{centering}
\end{table*}


==> tables/parallel-tests-table.tex <==
\begin{table}[h]
\begin{centering}
\tbl{Tests of the parallel regressions assumption for various model parameters. 
Test statistics for a $\chi^2$ distribution are shown.}{
\begin{tabular}{p{5cm} r r r}
\toprule
 & \multicolumn{1}{c}{$\chi^2$} & \multicolumn{1}{c}{$p < \chi^2$} & Degr. of Fr.\\[1ex]
 \cline{2-4}
Groupon mention      &  188.0890  &        0.000 & 3\\
Groupon user         & 1128.4384  &        0.000 & 3\\
Groupon period       &  810.1980  &        0.000 & 6\\
Review rank          &  477.4282  &        0.000 & 3\\
\bottomrule
\end{tabular}
}
\label{tab:ll-table}
\end{centering}
\end{table}


==> variables.tex <==
\newcommand{\numGrouponDeals}{16,692 }
\newcommand{\numGrouponBusinesses}{5,472 }
\newcommand{\numGrouponBusinessesLinked}{2,358 }
\newcommand{\numGrouponReviews}{251,681 }
\newcommand{\numNonGrouponReviewers}{127,946 }
\newcommand{\numGrouponReviewers}{21,020 }
\newcommand{\numGrouponReviewsComplete}{7,136,910 }
\newcommand{\numGrouponReviewersComplete}{148,966 }
\newcommand{\numGrouponBusinessesComplete}{942,589 }
\newcommand{\numGrouponReviewerOtherBusinesses}{464,706 }
\newcommand{\numGrouponReviewerOtherBusinessesSample}{25,128 }

